Designing IRS-Aided MIMO Systems for Secrecy Enhancement

Intelligent reflecting surfaces (IRSs) enable multiple-input multiple-output (MIMO) transmitters to modify the communication channels between the transmitters and receivers. In the presence of eavesdropping terminals, this degree of freedom can be used to effectively suppress the information leakage towards such malicious terminals. This leads to significant potential secrecy gains in IRS-aided MIMO systems. This work exploits these gains via a tractable joint design of downlink beamformers and IRS phase-shifts. In this respect, we consider a generic IRS-aided MIMO wiretap setting and invoke fractional programming and alternating optimization techniques to iteratively find the beamformers and phase-shifts that maximize the achievable weighted secrecy sum-rate. Our design concludes two low-complexity algorithms for joint beamforming and phase-shift tuning. Performance of the proposed algorithms are numerically evaluated and compared to the benchmark. The results reveal that integrating IRSs into MIMO systems not only boosts the secrecy performance of the system, but also improves the robustness against passive eavesdropping.

==> archive_of_writeup.tex <==
 we represent the direct equivalent channels from user $k$ and eavesdropper $j$ to the \ac{bs} by $\mh_{\rd, k} \in \setC^{M \times 1}$ and $\bgg_{\rd, j} \in \setC^{M \times 1}$, respectively. Similarly, the indirect channels from user $k$ and eavesdropper $j$ to the \ac{irs} are denoted by $\mh_{\rmr, k} \in \setC^{N \times 1}$ and $\bgg_{\rmr, j} \in \setC^{N \times 1}$, respectively, and $\mR\in \setC^{M \times N}$ is the channel matrix between the \ac{irs} to the \ac{bs}. The reflected signal received from the \ac{irs} is tuned by a diagonal phase shifting matrix modeled as $\mPhi= \diag\{\bphi\} $, where $\bphi=[\phi_1, \cdots, \phi_N]^\trp$ with $\phi_n$ being 
\begin{align}
	\phi_n=\beta_n e^{j \theta_n}.	
\end{align}
Here, $\beta_n \in [0, 1]$ denotes the amplitude reflection coefficient and $\theta_n\in [0, 2\pi ]$ is the phase shift applied by the $n$-th reflecting element of the \ac{irs}. We assume that $\beta_n=1$ for $\forall n \in N$ which means that the attenuation characteristics of all \ac{irs} elements are the same.


%%%%


The signal received at the legitimate user $k$ is written as 
\begin{align}
	{y}^\ell_k=\tilde{\mh}_k^\her (\bphi) \sum_{k=1}^K \bw_k s_k +z_k
\end{align}
where $z_k$ is additive white Gaussian noise at the $k$-th legitimate user with variance $\sigma_k^2$, i.e., $z_k \sim \mathcal{CN}(0, \sigma_k^2)$.


%%%%%%%5



At the \ac{bs} the transmitted signal $\bxx=[x_1, \cdots, x_M] ^\trp \in \setC ^{M \times 1}$ is constructed by  precoding  the vector of 


%%%%%%%%%%%%%%


 We first tackle the difficulty arising from the non-convex objective function by utilizing the closed-form \ac{fp} method recently introduced in \cite{ref2}. This approach deals with sum-fraction maximization problems and recast the original non-convex problem into a series of convex ones by introducing new auxiliary variables. Then, we make use of \ac{bcd} type algorithm to alternately solve the transformed problem with respect to various sets of optimization variables.
 
 
 %%%%%%%%%%
 
 \par By substituting $\sinr_k(\mW, \bphi)$ in \eqref{eq:sinr} and $\esnr_k(\mW, \bphi)$ in \eqref{eq:esnr} into the objective function of $\maP 2$, the optimization problem can be written as
 \begin{subequations}
 	\begin{align}
 		(\maP 3)&: \max _{\mW, \bphi, \mb} \quad \mar^\ssr_\rmq(\mW, \bphi, \mb)\overset{\Delta}{=}F_\ell(\mW, \bphi, \mb)+F_\ee(\mW, \bphi, \mb)\nonumber \\
 		\mathrm{s.t.} & \sum_{k=1}^K||\bw_k||^2\leq P_{\maxx}\label{eq:constraint1}\\ 
 		&\vert \phi_n \vert=1,~\forall n \in \{1, \cdots, N\}.
 		\label{eq:constraint23}
 	\end{align}
 \end{subequations}

%%%%%%%
Notice that the first term, i.e., $F_\ell(\mW, \bphi, \mb)$ is the weighted sum rate expression of a multi-user system without considering an eavesdropper. This term contains both fractional term and the logarithm operation, so it is not tractable. An equivalent amenable form of $F_\ell(\mW, \bphi, \mb)$  is derived in \cite{ref2} for a conventional multi-user system as an application of \ac{fp} approach in communication. Furthermore, by using the same approach, a tractable form of $F_{\ell}(\mW, \bphi, \mb)$ is determined in \cite{ref3} for an \ac{irs}-aided multi-user communication. 


Then, an equivalent form of $F_\ell(\mW, \bphi, \mb)$ is displayed in \eqref{eq:f1l} at the top of the next page where $\mbeta=[\alpha_1, \cdots, \alpha_K]^T$ and $\malpha=[\beta_1, \cdots, \beta_K]^T$ are sets of auxiliary variables \cite{ref3}.
\begin{figure*}[!t]
	\begin{align}\label{eq:f1l}
		\tilde{F}_{\ell}(\mW, \bphi, \malpha, \mbeta, \mb)=\sum_{k=1}^{K} b_k \left( \omega_{k}\Xi  (\alpha_k)
		+  2 \sqrt{\omega_{k}(1+\alpha_{k})} \operatorname{Re}\left\{\beta_{k}^* \tilde{\mh}^\her_k (\bphi) \bw_k\right\} - \left|\beta_{k}\right|^{2}\left(\sum_{i=1}^{K}\left|\tilde{\mh}^\her_k (\bphi) \bw_i\right|^{2}+\sigma_{k}^{2}\right)\right) .
	\end{align}
	\centering\rule{17cm}{0.1pt}
	\vspace*{2pt}
\end{figure*}
\par Leveraging \eqref{eq:f1l}, the optimization problem $\maP 3$ can be reformulated into the following problem
\begin{subequations}
	\begin{align}
		(\maP 4)&: \max _{\mW, \bphi, \malpha, \mbeta, \mb} \quad \mar^\ssr_\rmo(\mW, \bphi, \malpha, \mbeta, \mb)\nonumber \\
		\mathrm{s.t.} & \sum_{k=1}^K||\bw_k||^2\leq P_{\maxx}\label{eq:constraint1}\\ 
		&             \vert \phi_n \vert=1,~\forall n \in \{1, \cdots, N\}.
		\label{eq:constraint24}
	\end{align}
\end{subequations}
where 
\begin{align} \label{eq:Rssr}
	\mar^\ssr_\rmo(\mW, \bphi, \malpha, \mbeta, \mb)\overset{\Delta}{=}\tilde{F}_\ell(\mW, \bphi, \malpha, \mbeta, \mb)+F_\ee(\mW, \bphi, \mb)
\end{align}
\par The remaining difficulties in solving the optimization problem $\maP 3$ are left in the non-convex property of $F_\ee(\mW, \bphi, \mb)$ and unit modulus-constraint of \eqref{eq:constraint24}. In this paper, we propose using the Lagrangian dual transform \cite{ref5} to tackle the difficulty arising from the the ratio terms inside the logarithm function of $F_\ee(\mW, \bphi, \mb)$. Before proceeding, let us briefly introduce this theorem in the sequel.


In the following, the \ac{bcd} algorithm is used to alternately maximize $\mar^\ssr_\rmo$ with respect to variables $\mW$, $\bphi$, $\mb$, $\malpha$ and $\mbeta$. Specifically, we update one variable in each step while keeping the the other variables fixed. This leads to the following subproblems in each \ac{bcd} iteration.
%%-------------------------------------------------------------------------------%%
\par \emph{1) The subproblem w.r.t to the precoding Matrix $\mW$:} Here, we focus on optimizing the precoding matrix $\mW$ while the other variables are held fixed.  For a given $\bphi$, $\mb$, $\malpha$ and $\mbeta$, the only non-convexity of the problem $\maP 3$ with respect to $\mW$ is due to the fractional $\esnr$ term inside the logarithm operation. To overcome this challenge, we adopt the Lagrangian dual transform technique to move the ratio term to the outside of the logarithm function. Here, the application of Lagrangian dual transformation to $F_\ee(\mW, \bphi, \mb)$ is not as straightforward as convex reformulation of $F_\ell(\mW, \bphi, \mb)$ derived in \cite{ref3}. Since the argument of $F_\ee(\mW, \bphi, \mb)$ is less than 1, the Lagrangian dual transform can not be employed directly. In order to write $F_\ee(\mW, \bphi, \mb)$ as a standard form of \eqref{eq:Lag}, we first apply the relaxation trick \cite{ref4} to $F_\ee$, which reads
\begin{align}\label{eq:relaxation-trick}
	\frac{1}{1+||\mathbf{\Upsilon}_{\ee}\mathbf{\tilde{G}^\her}(\bphi)\bw_k||^2}\leq \frac{1}{1+||\mathbf{\Upsilon}_{\ee}\mathbf{\tilde{G}^\her}(\bphi)||^2 P_{\maxx}}.
\end{align}
By plugging \eqref{eq:relaxation-trick} into \eqref{eq:fee}, $F_\ee(\mW, \bphi, \mb)$ is equivalently written as
\begin{align}\nonumber
	&F_{1 \ee}(\mW, \bphi, \mb)=\\ &\sum_{k=1}^{K} \omega_k b_k\log\left( \frac{1+||\mathbf{\Upsilon}_{\ee}\mathbf{\tilde{G}^\her}(\bphi)||^2P_{\maxx}}{1+||\mathbf{\Upsilon}_{\ee}\mathbf{\tilde{G}^\her}(\bphi)\bw_k||^2}\right) - C_{\esnr}
\end{align}
with $C_{\esnr}$ being defined as follows
\begin{align}
	C_{\esnr}=\sum_{k=1}^{K} \omega_k b_k\log\left(1+||\mathbf{\Upsilon}_{\ee}\mathbf{\tilde{G}^\her}(\bphi)||^2 P_{\maxx}\right).
\end{align}
By introducing the auxiliary variable $\malpha_\ee$ defined as $\malpha_\ee=[\alpha_{\ee 1}, \cdots, \alpha_{\ee K}]^T$ and utilizing the Lagrangian dual transform technique in theorem 1, an equivalent form of $F_{1 \ee}(\mW, \bphi, \mb)$ can be written as $\tilde{F}_{\ee}(\mW, \malpha_\ee, \mb)$ displayed in \eqref{eq:fee_equ} at the top of the next page. 
\begin{figure*}[!t]
	\begin{align}\label{eq:fee_equ}
		\tilde{F}_{\ee}(\mW,  \bphi, \malpha_\ee, \mb)=\sum_{k=1}^{K} \omega_{k} b_k \left(  \Xi(\alpha_{\ee k}) +  (1+\alpha_{\ee k}) \dfrac{ ||\mathbf{\Upsilon}_{\ee}\mathbf{\tilde{G}}(\bphi)||^2P_{\maxx}- ||\mathbf{\Upsilon}_{\ee}\mathbf{\tilde{G}}(\bphi)\bw_k||^2}{1+||\mathbf{\Upsilon}_{\ee}\mathbf{\tilde{G}}(\bphi)||^2P_{\maxx}}\right) - C_{\esnr}
	\end{align}
	\centering\rule{17cm}{0.1pt}
	\vspace*{2pt}
\end{figure*}
By inserting \eqref{eq:fee_equ} into objective function of the problem $\maP 4$ and dropping the constant terms, the precoding optimization problem can be equivalently written as
\begin{subequations}
	\begin{align}\nonumber
		(\maP 5):\max _{\mW, \malpha_\ee}\sum_{k=1}^{K} &\nu_k \operatorname{Re}\left\{\beta_{k}^* \tilde{\mh}^\her_k (\bphi) \bw_k\right\} - b_k \left|\beta_{k}\right|^{2}\sum_{i=1}^{K}\left|\tilde{\mh}^\her_k (\bphi) \bw_i\right|^{2}\\&-
		\rho_k(1+\alpha_{\ee k})||\mathbf{\Upsilon}_{\ee}\mathbf{\tilde{G}^\her}(\bphi)\bw_k||^2+\kappa_k(1+\alpha_{\ee k})~\nonumber \\
		&+\tau_k\Xi(\alpha_{\ee k})\label{eq:p5}\\
		\mathrm{s.t.}& \quad \sum_{k=1}^K||\bw_k||^2\leq P_{\maxx}
		\label{eq:constraintw}
	\end{align}
\end{subequations}
where the parameters in \eqref{eq:p5} are defined as
\begin{align}
	\nu_k&\overset{\Delta}{=} 2 b_k \sqrt{\omega_{k}(1+\alpha_{k})},\label{eq:upsilon}\\
	\tau_k&\overset{\Delta}{=}\omega_{k} b_k\label{eq:tau}\\
	\rho_k&\overset{\Delta}{=}\dfrac{\tau_k}{1+||\mathbf{\Upsilon}_{\ee}\mathbf{\tilde{G}^\her}(\bphi)||^2P_{\maxx}}\\
	\kappa_k&\overset{\Delta}{=}\rho_k ||\mathbf{\Upsilon}_{\ee}\mathbf{\tilde{G}^\her}(\bphi)||^2P_{\maxx}.\label{eq:rho}
\end{align}
Note that the problem $\maP 5$ has a biconvex objective function with a convex constraint which enables us to adopt a 2-block \ac{bcd} algorithm and cyclically optimize $\mW$ and $\malpha$. Specifically, when $\alpha$ is given, the problem $\maP 5$ with respect to $\mW$ is a quadratic optimization problem with power constraint. By applying the first order optimality condition, we can obtain the following closed-form solution for $\bw_k$ as follows
\begin{align}
	\bw_k^{\opt}=\nu_k \beta_k\left( \zeta \mI_M+\mA_k\right) ^{-1} \tilde{\mh}_k(\bphi) \label{eq:wopt}
\end{align}
with the  matrix $\mA_k$ being defined as
\begin{align}
	\mA_k=\rho_k(1+\alpha_{\ee k}) \mathbf{\tilde{G}}(\bphi)\mathbf{\Upsilon}_{\ee}^2\mathbf{\tilde{G}^\her(\bphi)}+b_k \sum_{i=1}^K|\beta_i^2| \tilde{\mh}_i(\bphi) \tilde{\mh}^\her_i(\bphi) 
\end{align}
with $\zeta$ being the non-negative Lagrange multiplier for the power constraint \eqref{eq:rho}, which can be efficiently determind by utilizing the bisection method as
\begin{align}
	\sum_{k=1}^{K}\Tr\left( \nu_k^2 \beta_k^2\tilde{\mh}_k^\her(\bphi)\left( \zeta \mI_M+\mA_k\right) ^{-2} \tilde{\mh}_k(\bphi)\right) = P_\maxx.
\end{align}


\par When $\mW$ is given, by dropping the constant terms independent of $\malpha_{\ee}$ in $\maP 5$, the optimal $\malpha_{\ee}$ can be obtained as
\begin{align}
	\alpha_{\ee k}=\arg &\max_{\malpha_\ee}
	\kappa_k(1+\alpha_{\ee k})
	+\tau_k\Xi(\alpha_{\ee k})\nonumber\\&-
	\rho_k(1+\alpha_{\ee k})||\mathbf{\Upsilon}_{\ee}\mathbf{\tilde{G}^\her}(\bphi)\bw_k||^2\nonumber\\
	&=\dfrac{ ||\mathbf{\Upsilon}_{\ee}\mathbf{\tilde{G}^\her}(\bphi)||^2P_{\maxx}- ||\mathbf{\Upsilon}_{\ee}\mathbf{\tilde{G}^\her}(\bphi)\bw_k||^2}{1+||\mathbf{\Upsilon}_{\ee}\mathbf{\tilde{G}^\her}(\bphi)\bw_k||^2}\label{eq:alpha-e}
\end{align}
%------------------------------------------------------------------------------%

With respect to $\bphi$, the difficulties in solving problem $\maP 4$ lies in the non-convexity of $F_\ee$ in the objective function and the presence of the unit-modulus constraint. In order to find a tractable solution, we first reformulated the objective function in a tractable form and then we propose two algorithms to derive a closed form solution for the phase-shifting matrix.

%=================
where $\tilde{C}_{\esnr}=\log\left( 1+ \esnr_k^\mathcal{U}(\mW, \bphi) \right)$. Now, the reformulated $F_{2 \ee}(\mW, \bphi, \mb)$ satisfies the conditions for applying the Lagrangian dual transform. Hence, by dropping the constant terms in \eqref{eq:trnsF_e}, $F_{2 \ee}(\mW, \bphi, \mb)$ can be equivalently transformed to
\begin{align}\label{eq:trnsf_e}
	&\hat{F}_{\ee}(\mW, \bphi, \mgamma, \mb)=\nonumber\\&\sum_{k=1}^{K} \omega_{k} b_k \left( \Xi(\gamma_k) +  (1+\gamma_{k}) \dfrac{\esnr_k^\mathcal{U}- \esnr_k(\mW, \bphi)}{1+\esnr_k^\mathcal{U}}\right)
\end{align}
where $\mgamma=[\gamma_1, \cdots, \gamma_K]^\trp$ is a vector of auxiliary variables.
\par Thus,  by dropping the constant terms and inserting \eqref{eq:trnsf_e} into \eqref{eq:Rssr}, the optimization problem $\maP 4$ is recast to
%\par Upon substituting \eqref{eq:htrnsf} into \eqref{eq:f1l} and dropping the constant terms, the optimization problem $\maP 4$ over $\bphi$ can equivalently transformed to the following optimization problem over $\bphi$ and $\gamma$
\begin{subequations}
	%############################
	\begin{align}\nonumber
		(\maP 6): \max _{\bphi, \gamma}\sum_{k=1}^{K} &\nu_k \operatorname{Re}\left\{\beta_{k}^* \tilde{\mh}^\her_k (\bphi) \bw_k\right\} - b_k \left|\beta_{k}\right|^{2}\sum_{i=1}^{K}\left|\tilde{\mh}^\her_k (\bphi) \bw_i\right|^{2}\\
		&-\iota_k\left( 1+\gamma_k\right) \sum_{j=1}^J  \dfrac{1}{\mu_j^2}\vert \bgg_{\rd, j}^\her \bw_k + \bphi^\her \mG_j^\her \bw_k  \vert^2 \nonumber \\
		&+\varpi_k \left( 1+\gamma_k\right)+\tau_k \Xi(\gamma_k)\label{eq:phi-trns}\\
		\mathrm{s.t.}& \quad  \vert \phi_n \vert=1,~\forall n \in \{1, \cdots, N\}
		\label{eq:constraintphi}
	\end{align}
\end{subequations}	
where $\iota_k$ and $\varpi_k$ are respectively given by
\begin{align}
	\iota_k&\overset{\Delta}{=}\dfrac{\omega_k b_k}{1+\esnr_k^\mathcal{U}}\\
	\varpi_k&\overset{\Delta}{=}\iota_k\esnr_k^\mathcal{U}
\end{align}
with $\nu_k$ and  $\tau_k$ being defined in \eqref{eq:upsilon} and \eqref{eq:tau}, respectively. Thanks to the Lagrangian dual transform, the logarithm expression and ratio terms have been removed in \eqref{eq:phi-trns} compared with the objective function of the problem $\maP 4$. However, the the problem $\maP 6$ with respect to $\bphi$ is still non-convex due to the unit-modulus constraint \eqref{eq:constraintphi}. In the following, we adopt a 2-block \ac{bcd} algorithm to solve the problem $\maP 6$ which cyclically updates $\gamma$ and $\bphi$ until convergence is achieved. First, assume $\bphi$ is a given fixed constant, the optimal $\gamma$ can be accordingly obtained by solving the following subproblem
\begin{align}\nonumber
	\gamma_k&=\arg\max _{\mgamma}\sum_{k=1}^{K} -\iota_k\left( 1+\gamma_k\right) \sum_{j=1}^J  \dfrac{1}{\mu_j^2}\vert \bgg_{\rd, j}^\her \bw_k + \bphi^\her \mG_j^\her \bw_k  \vert^2 \nonumber \\
	&+\varpi_k \left( 1+\gamma_k\right)+\tau_k \Xi(\gamma_k)\nonumber\\
	&=\dfrac{\esnr_k^\mathcal{U}-\esnr_k(\mW, \bphi)}{1+\esnr_k(\mW, \bphi)}\label{eq:Gamma}
\end{align}


\par \emph{3) The subproblem w.r.t to auxiliary set ${\malpha}$:}
We now turn our attention to optimize the auxiliary variable ${\malpha}$. For a given $\left(\mW, \bphi, \mb, \mbeta\right)$, by dropping the constant terms in problem $\maP 4$, the subproblem with respect to $\malpha$ is equivalent to
\begin{align}\nonumber
	\alpha_k&=\arg\max _{\malpha}\sum_{k=1}^{K} \tau_k \Xi  (\alpha_k)  
	+  4 b_k \sqrt{\omega_{k}(1+\alpha_{k})} \chi_k \\
	&=2\omega_k^{-1}\chi_k\left( \chi_{k} + \left(\chi_k^2+\omega_k \right)^{\frac{1}{2}} \right) \label{eq:alpha}
\end{align}
where $\chi_k=\dfrac{1}{2}\operatorname{Re}\left\{\beta_{k}^* \tilde{\mh}^\her_k (\bphi) \bw_k\right\}$.

%--------------------------------------------------------------------------------%
\par \emph{4) The subproblem w.r.t to auxiliary set ${\mbeta}:$}
Similarly, while fixing the other variables and dropping the irrelevant constant terms of the problem $\maP 4$, the subproblem with respect to $\mbeta$ can be expressed as
\begin{align}
	\label{eq:beta_up}
	\max _{\mbeta} \sum_{k=1}^K \nu_k\operatorname{Re}\left\{\beta_{k}^* \tilde{\mh}^\her_k (\bphi) \bw_k\right\} - b_k\left|\beta_{k}\right|^{2}\left(\sum_{i=1}^{K}\left|\tilde{\mh}^\her_k (\bphi) \bw_i\right|^{2}+\sigma_{k}^{2}\right)
\end{align}
which is convex and the optimal $\beta_k$ is given as follows
\begin{align}\label{eq:betta}
	\beta_k=\dfrac{\sqrt{\omega_k \left( 1+\alpha_k\right) }\tilde{\mh}^\her_k (\bphi) \bw_k}{\sum_{i=1}^{K}\left|\tilde{\mh}^\her_k (\bphi) \bw_i\right|^{2}+\sigma_{k}^{2}}
\end{align}
%----------------------------------------------------------------------------------
By replacing $\tilde{\mh}_k \brc{\bphi}$ with its definition, we have


$\mh_{\rd, k}+\mF_k \bphi$ into \eqref{eq:phi-trns} and ignoring the terms independent of $\bphi$, the problem $\maP 6$ can be equivalently represented as
\begin{subequations}
	\begin{align}
		(\maP 7): \max _{\bphi} &~\Omega(\bphi)= -\bphi^\her \mQ\bphi+2\operatorname{Re}\left\lbrace \bphi^\her \mq \right\rbrace \label{eq:phi}\\
		\mathrm{s.t.}& \quad  \vert \phi_n \vert=1,~\forall n \in \{1, \cdots, N\}\label{eq:constP7}
	\end{align}
\end{subequations}
where the parameters $\mQ$ and $\mq$ are defined as
\begin{subequations}
	\begin{align}
		\mR_k&\overset{\Delta}{=}\sum_{i=1}^K \mF_k^\her\bw_i \bw_i^\her \mF_k, ~ \mU_k\overset{\Delta}{=}\sum_{j=1}^{J} \dfrac{1}{\mu_j^2} \mG_j^\her \bw_k \bw_k^\her \mG_j\\
		\mQ&\overset{\Delta}{=}\sum_{k=1}^K b_k \vert \beta_{k}\vert^2 \mR_k+\iota_k\left( 1+\gamma_k\right) \mU_k\\
		\mathbf{r}_k&\overset{\Delta}{=}\sum_{i=1}^{K} \mF_k^\her\bw_i \bw_i^\her \mh_{\rd, k}, ~ \mathbf{u}_k\overset{\Delta}{=} \sum_{j=1}^{J} \dfrac{1}{\mu_j^2}\mG_j^\her \bw_k \bw_k^\her \mathbf{g}_{\rd, j}\\ 
		\mathbf{q}&=\sum_{k=1}^{K}\frac{\nu_k}{2}\beta_k^*\mF_k^\her\bw_k-b_k \vert \beta_{k}\vert^2\mathbf{r}_k-\iota_k\left( 1+\gamma_k\right)\mathbf{u}_k
	\end{align}
\end{subequations}
The main difficulty in solving the problem $\maP 7$ is caused by the non-linear unit-modulus constraint of \eqref{eq:constP7}. To address this challenge, we apply two algorithms for solving this issue.
\par \emph{A) \ac{mm} Method:} 
\par \textcolor{red}{Here comes a brief description of MM algorithm.}
\par In this subsection, we develop an algorithm for solving the problem $\maP 7$ via \ac{mm} technique.


\begin{algorithm} 
	
	\begin{algorithmic}[1]
		\renewcommand{\algorithmicrequire}{\textbf{Input:}}
		\renewcommand{\algorithmicensure}{\textbf{Output:}}
		\REQUIRE Initial $\bphi^{\left( 0\right)} $, $\mQ$, $\mq$, $\mP$ and $t=0$;
		\STATE define $\tilde{\mQ}= \mP^\her \mQ \mP$ and $\tilde{\mq}=\mP^\her \mq$ 
		\STATE set $\tilde{q}_1$ and $\tilde{\mq}_{21}$ as
		\begin{align}
			\tilde{\mQ}=
			\begin{bmatrix}
				\tilde{q}_{11} & \tilde{\mq}_{21}^\her \\
				\tilde{\mq}_{21} & \tilde{\mQ}_{22}
			\end{bmatrix},
			~\tilde{\mq}=\left[\tilde{q}_1; \bar{\mq}\right] \label{eq:Qtild}	
		\end{align}
		%\ENSURE  out
		%\\ \textit{Initialisation} :
		%%%%
		\STATE \textbf{repeat:}
		\FOR {$n = 1$ to $N$}
		\STATE set $\bar{\bphi}^{\left( t \right) }=[\phi_1^{\left( t \right) }, \cdots, \phi_{n-1}^{\left( t \right) }, \phi_{n+1}^{\left( t \right) }, \cdots, \phi_N^{\left( t \right) }]^\trp$
		\STATE set $\eta=\left(\tilde{q}_1^*- {\left( \bar{\bphi}^{\left( t \right) }\right) }^\her\tilde{\mq}_{21} \right)^*$
		\STATE Update $\phi_n^{\left( t+1 \right) }=\frac{\eta}{\vert \eta \vert}$
		\ENDFOR
		\STATE $t \leftarrow t+1$
		%%%%%
		\STATE \textbf{until} convergence
	\end{algorithmic} 
\end{algorithm}


\section{The Proof of Lemma~\ref{Lemma:2}}
\label{app:Lem2}
Let $\mP_n$ be a permutation matrix constructed by moving the $n$-th column vector of the identity matrix to the first column. This means that the permuted vector $\tilde{\bphi} = \mP_n^\her \bphi $ is of the form
\begin{align}
	\tilde{\bphi}= \dbc{ \phi_n, \phi_1, \ldots, \phi_{n-1}, \phi_{n+1}, \ldots, \phi_N}^\trp.
\end{align}
Moreover, we define $\tilde{\mQ}= \mP^\her \mQ \mP$ and $\tilde{\mq}=\mP^\her \mq$. Then, $\Omega(\bphi)$ can be written as
\begin{align}
	\Omega(\bphi)&= -\bphi^\her \mQ\bphi+2\operatorname{Re}\left\lbrace \bphi^\her \mq \right\rbrace \nonumber\\
	&= -\tilde{\bphi}^\her \mP^\her \mQ \mP \tilde{\bphi}+2\operatorname{Re}\left\lbrace \tilde{\bphi}^\her\mP^\her \mq \right\rbrace \nonumber\\
	&= -\tilde{\bphi}^\her \tilde{\mQ} \tilde{\bphi}+2\operatorname{Re}\left\lbrace \tilde{\bphi}^\her\tilde{\mq} \right\rbrace\nonumber\\
	&\overset{\dagger}{=} -\tilde{\bphi}^\her \tilde{\mQ} \tilde{\bphi}+2\operatorname{Re}\left\lbrace \tilde{\mq}^\her\tilde{\bphi} \right\rbrace \label{eq:phit}
\end{align}
where $\dagger$ comes from the fact that $\operatorname{Re}\left\lbrace \mff^\her\mgg \right\rbrace=\operatorname{Re}\left\lbrace \mgg^\her\mff \right\rbrace$. Furthermore, $\tilde{\mQ}$ and $\tilde{\mq}$ can be expressed as
\begin{align}
	\tilde{\mQ}=
	\begin{bmatrix}
		\tilde{q}_{11} & \tilde{\mq}_{21}^\her \\
		\tilde{\mq}_{21} & \tilde{\mQ}_{22}
	\end{bmatrix},
	~\tilde{\mq}=\left[\tilde{q}_1; \bar{\mq}\right] \label{eq:Qtild}	
\end{align}
where $\bar{\mq}=\left[ \tilde{q}_2, \cdots, \tilde{q}_N\right] $. By substituting \eqref{eq:Qtild} into \eqref{eq:phit} and following some mathematical manipulations, $\Omega(\bphi)$ can be rearranged as follows
\begin{align}
	\Omega(\bphi)=\delta\vert \phi_n \vert ^2 + 2\operatorname{Re}\left\lbrace \eta^* \phi_n \right\rbrace +\varrho 
\end{align}
with $a$, $b$ and $c$  being defined as
\begin{align}
	\delta&=-\tilde{q}_{11} \label{eq:delta}\\
	\eta&=\left(\tilde{q}_1^*- \bar{\bphi}^\her\tilde{\mq}_{21} \right)^* \label{eq:eta}\\
	\varrho&=-\bar{\bphi}^\her \tilde{\mQ}_{22} \bar{\bphi}+2\operatorname{Re}\left\lbrace \bar{\bphi}^\her \bar{\mq} \right\rbrace\label{eq:varrho}.
\end{align} 
